Decoupling Precipitation and Surface Complexation during Mn(II) Removal by Biochar via Experiments and Atomistic Simulations

Manganese(II) mobilised by mining activity poses a persistent water-quality challenge, yet the mechanisms by which low-cost sorbents, such as biochar, sequester Mn(II) remain poorly resolved. This study identifies the specific chemical drivers of Mn(II) sequestration by combining fixed-bed column and batch experiments with atomistic molecular dynamics simulations. Oilseed rape straw biochars, produced at 350\textdegree C, 550\textdegree C, and 700\textdegree C, removed 20-50% of dissolved Mn from acidic influent (pH 4, 5 ppm). High-temperature biochar achieved the greatest removal ($\sim$50%) and rapidly increased effluent pH to 9, triggering alkaline precipitation. Conversely, lower-temperature biochars removed 20-30% of Mn while maintaining a near-neutral pH (7-7.5). Enhanced \ce{K+} release in these systems indicates significant cation exchange and non-precipitative pathways. Molecular simulations confirmed that while neutral surfaces show weak Mn(II) association, deprotonated sites drive strong adsorption through inner-sphere complexation ($\sim$50% removal) and outer-sphere association ($\sim$10%). These results establish a mechanistic framework to distinguish between precipitation-led and surface-complexation-led removal. By providing specific chemical criteria for Mn-targeted sequestration, this work enables the rational design of engineered biochars for sustainable water remediation.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
